Factorizing the factorization - a spectral-element solver for elliptic equations with linear operation count

High-order methods gain more and more attention in computational fluid dynamics. However, the potential advantage of these methods depends critically on the availability of efficient elliptic solvers. With spectral-element methods, static condensation is a common approach to reduce the number of degree of freedoms and to improve the condition of the algebraic equations. The resulting system is block-structured and the face-based operator well suited for matrix-matrix multiplications. However, a straight-forward implementation scales super-linearly with the number of unknowns and, therefore, prohibits the application to high polynomial degrees. This paper proposes a novel factorization technique, which yields a linear operation count of just 13N multiplications, where N is the total number of unknowns. In comparison to previous work it saves a factor larger than 3 and clearly outpaces unfactored variants for all polynomial degrees. Using the new technique as a building block for a preconditioned conjugate gradient method resulted in a runtime scaling linearly with N for polynomial degrees $2 \leq p \leq 32$ . Moreover the solver proved remarkably robust for aspect ratios up to 128.

==> solver_po_alpha_1.0_cputime_per_dof.tex <==
\begin{tabular}{rrrrrrrrrrr}
\toprule
&&&& \multicolumn{7}{c}{Solution time per DOF \mbox{$[\mathrm{\mu s}]$}}\\
\cmidrule{5-11}$p$ & \phantom{a} & $n_\mathrm{DOF}$ & \phantom{a} & UC & \phantom{a} & DC & \phantom{a} & BC & \phantom{a} & BT\\ \midrule
8 && -127 && -12001.34 && -11400.38 && -10629.54 && -3760.32\\
12 && -331 && -14642.69 && -13419.96 && -11895.26 && -5025.96\\
16 && -631 && -20270.16 && -18130.32 && -14530.29 && -6416.15\\
20 && -1027 && -27349.64 && -23957.88 && -18710.63 && -7853.68\\
24 && -1519 && -35165.80 && -30598.29 && -22586.84 && -8789.80\\
28 && -2107 && -41815.96 && -36066.37 && -25853.15 && -9714.90\\
32 && -2791 && -48920.53 && -41899.21 && -28888.37 && -10891.33\\
\bottomrule
\end{tabular}


==> solver_po_alpha_1.0_itertime_per_dof.tex <==
\begin{tabular}{rrrrrrrrrrr}
\toprule
&&&& \multicolumn{7}{c}{Appr. iteration time per DOF \mbox{$[\mathrm{ns}]$}}\\
\cmidrule{5-11}$p$ & \phantom{a} & $n_\mathrm{DOF}$ & \phantom{a} & UC & \phantom{a} & DC & \phantom{a} & BC & \phantom{a} & BT\\ \midrule
8 && -127 && -75957.8 && -81431.3 && -109582.8 && -38370.6\\
12 && -331 && -71427.8 && -77572.0 && -103437.1 && -43704.0\\
16 && -631 && -82399.0 && -88440.6 && -116242.3 && -50921.8\\
20 && -1027 && -98027.4 && -102823.5 && -139631.6 && -57747.7\\
24 && -1519 && -112350.8 && -119059.5 && -162495.3 && -61900.0\\
28 && -2107 && -122268.9 && -128808.5 && -177076.4 && -65641.2\\
32 && -2791 && -132576.0 && -139200.0 && -191313.7 && -71185.2\\
\bottomrule
\end{tabular}

